Targeted Adversarial Training for Natural Language Understanding

We present a simple yet effective Targeted Adversarial Training (TAT) algorithm to improve adversarial training for natural language understanding. The key idea is to introspect current mistakes and prioritize adversarial training steps to where the model errs the most. Experiments show that TAT can significantly improve accuracy over standard adversarial training on GLUE and attain new state-of-the-art zero-shot results on XNLI. Our code will be released at: https://github.com/namisan/mt-dnn.

==> 1_intro_v2.tex <==
Although deep learning models have been very successful in various kinds of NLP
problems, they are known to be sensitive towards input data distribution change
����which are pervasive across language tasks.
Motivated by this, a recent line of work investigate the adversarial training
technique to enhance the model robustness.
Most existing methods focus on generating \textit{adversarial} examples by
adding small perturbations to original clean examples based on the \textit{local}
curvature of the corresponding loss function.
Typically, the perturbation direction is chosen to mislead the model to flip the
correct output to an arbitrary wrong one at the instance level.
However, this local strategy might not be optimal because it does not make use
of \textit{global} knowledge of output label relation during the search.
Therefore, in this work, we aim to investigate the use of global knowledge of
labels for adversarial training.

There are many types of label information that can be potentially useful for
guiding the adversarial training.
In general, they can be categorized into
1) model-based label relation: model confusion, or variability;
2) task-specific label relation: class hierarchy;
3) dataset label relation: annotator agreement, and label imbalance.
Here, we mainly focus on exploring the label confusion to guide 
the search for better perturbations during adversarial training.
For example, on the MNLI dataset, classifiers
often misclassify the samples with the true label ``entailment'' as ``neutral''
rather than ``contradiction'', while samples with the true label
``contradiction'' are more often missclassified as ``neutral'' rather than
``entailment'' (based on the confusion matrix on the development set as shown in
Figure~\ref{fig:cmt} (a)).
Based on this observation, we propose to generate more informative adversarial
perturbations by fooling the model to flip the prediction to the corresponding
confusable one.
We compare our proposed TAT with existing popular adversarial training methods
over a wide range of text classification tasks.
Our results indicate that the proposed target-based method can significantly
improve model performance over BERT-based baselines on the GLUE benchmark.
Additionally, compared with other adversarial training methods, TAT lead to
superior model transferability in terms of data bias, domain shift, and more remarkably
cross-lingual scenario.
In sum, the contributions of this paper are as follows:
\begin{enumerate}
	\item We propose a new method of guiding the adversarial training with
		\textit{global} label confusion information.
	\item We demonstrate that the proposed method can lead to better model accuracy
		and robustness on a wide range of text classification tasks.
	\item We advance the state-of-the-art accuracy on XNLI zero-shot setting.
\end{enumerate}


==> 3_model.tex <==
% !TEX encoding = UTF-8
% !TEX Root = Main.tex
\section{Model}
\label{sec:model}
Given its superior performance over a wide range of NLP tasks, we focus on exploring different training techniques using BERT \cite{devlin2018bert}. 
We first describe the BERT representations used for all tasks considered in this paper. 
Then, two variants of task-specific BERT-based models are introduced: 
1) the sentence-level classifier for textual entailment and sentiment analysis,
and 2) the extractive QA model.
Specifically, we focus on different ways of encoding input text and building task-specific layers using BERT representations.

\subsection{BERT Representation}

For all tasks considered in this work, an input text sequence is divided into subword units $w_t, t=1, \ldots, T$.
The tokenized input sequence is then transformed into embeddings, $\xvec_1, \ldots, \xvec_T\in\RR^n$, through a token encoder, which combines 
a token embedding, a (token) position embedding and a segment embedding (i.e., which text span the token belongs to) by element-wise summation.
The embedding layer is used as the input to multiple transformer layers \cite{vaswani2017attention} to generate the contextual representations, $\hvec_1, \ldots, \hvec_T\in\RR^d$, which are the hidden states of the last layer of the BERT model.
For all robust learning techniques, we sample noise vectors $\epsilon_1, \ldots, \epsilon_T$ from $\mathcal{N}(0, c^2I)$, 
and add them to the token embeddings as the noisy input, \ie $\xvec_1+\epsilon_1, \ldots, \xvec_T+\epsilon_T$.

\subsection{Sentence-level Classifier}
Following the standard setup of BERT-based textual entailment model \cite{devlin2018bert}, a pair of premise and hypothesis is converted into an input sequence in the form of "\clstoken \textit{premise} \septoken \textit{hypothesis} \septoken". %\todo{ending \septoken?}
Here, \clstoken is a special token indicating the start of the whole sequence and \septoken is another special token for separating the two sentences.
For sentiment analysis, a single sentence is converted to the form of
"\clstoken \textit{sentence} \septoken". 

For both textual entailment and sentiment analysis, the task-specific layer only takes the first hidden vector $\hvec_{[CLS]}$ produced by BERT, 
corresponding to the \clstoken token.
Then, the probability of class $k$ is
\begin{align}
\label{eqn:class_obj}
P(k|w_1, \ldots, w_T) \propto W^C_k \hvec_{[CLS]},
\end{align}
where $W^C\in\RR^{m\times d}$ is the learnable parameter, the subscript $k$ indicates the $k$-th row of the matrix, and the bias term is left out for simplicity.

For standard BERT training, the log-likelihood based on \autoref{eqn:class_obj} is maximized. For robust learning methods, the regularization term is imposed to stabilize the class probability change with regard to the input noise.

\subsection{Extractive QA Model}
For extractive QA, the probability space outcomes consist of token positions of answer spans.
Given a pair of question $q$ and a passage $p$ in the form of "\clstoken \textit{question} \septoken \textit{passage} \septoken",
the BERT encoder produces contextualized representations for all tokens in the input.
Specifically, for each token position $t$ in $p$,
the final hidden vector $\hvec_t \in \RR^d$ 
is used as the contextualized token embedding, where $d$ is the vector dimension.

The span-begin score is computed as 
$s_b(i) = \wvec_b^T \hvec_i$ using a weight vector
$\wvec_b \in \RR^d$.
% The span-end score $s_e(j)$ is defined in the same way.
% The probabilities for a start position $i$ and an end position $j$ are
% \begin{eqnarray}
% \label{eqn:span_begin_prob}
% P_b(i) = {\exp(s_b(i)) \over Z_b},\\
% \label{eqn:span_end_prob}
% P_e(j) = {\exp(s_e(j)) \over Z_e},
% \end{eqnarray}
% where $Z_b$ and $Z_e$ are normalizing factors computed by normalizing over all possible positions, i.e.,
% \begin{align}
% \label{eqn:par_begin_z}
%     Z_b = \sum_{i \in \mathcal{I}} \exp (s_b(i)), \\
% \label{eqn:par_end_z}
%     Z_e = \sum_{j \in \mathcal{I}} \exp (s_e(j)),
% \end{align}
% where $\mathcal{I}$ is the set of all positions in the passage. 
The probability for a start position $i$ is

Maximizing the log-likelihood of the above equation is equivalent to maximizing the log probabilities for the correct start and end position, respectively.
For all robust learning techniques, given it is computationally expensive to enumerate all possible spans, we apply two separate regularization terms for the start and end position probabilities, respectively.



==> 4-exp-old.tex <==
% !TEX encoding = UTF-8
% !TEX Root = Main.tex

\section{Experiments}
\label{sec:exp}
We compare the proposed TAT with recent adversarial training methods in terms of their generalization ability over both in-domain and out-of-domain evaluation sets.
Specifically, we first apply different adversarial training methods on top of BERT \cite{devlin2018bert} over GLUE benchmark \cite{wang2018glue} for comparing model in-domain generalization ability.
In addition, we evaluate the robustness of different MNLI \cite{mnli2018} models trained with different training approaches to a set of out-of-domain NLI datasets \cite{snli2015,mccoy2019hans,scitail,romanov2018mednli}.
Lastly, we study the application of our TAT method to a zero-shot cross-lingual transfer learning setting with XNLI \cite{conneau2018xnli}.

% We mainly evaluate TAT on the GLUE \cite{wang2018glue} benchmark, which is a collection of
% nine NLU tasks. The diversity of the tasks makes GLUE very suitable for evaluating the generalization and robustness of NLU models. We also use SNLI \cite{snli2015}, SciTail \cite{scitail}, HANS \cite{mccoy2019hans} and MedNLI \cite{romanov2018mednli} for assessing model generalization. At last, XNLI \cite{conneau2018xnli} is used for assessing domain transformation in multilingual settings. Due to space limitations, detailed descriptions of the datasets can be found in Appendix~\ref{sec:appendix} and implementation details are reported in Appendix~\ref{sec:param}.
 
\subsection{GLUE main results}
\label{subsec:glue}
In this part, we carry out experiments on the GLUE benchmark and a collection of out-of-domain NLI evaluation sets.
Given its superior performance over a wide range of NLP tasks, we consider the application of different adversarial training methods on top of the pre-trained uncased BERT-base model \cite{devlin2018bert}.
Here, we compare the proposed TAT with the following baselines:

% We first evaluate TAT on the GLUE benchmark. All experiments are based on the pre-trained BERT-base uncased model \cite{devlin2018bert}, which includes 110M parameters, since it is widely used in NLU tasks. For the sake of simplicity, we drop BERT. We compare TAT to the following baseline models.
\begin{enumerate}
    %\item \textbf{STD}: the standard BERT fine-tuning results from \cite{devlin2018bert}.
    %\hao{Do we need this? If not, then all results are from our implementation. We don't have to clairfy which is re-implemented. Also, we need to have some discussion over the difference between VAT and FreeLB, such as one if using the original classification loss but the other is using logits difference.}
    \item \textbf{STD}: the standard BERT training.
    \item \textbf{FreeLB}: the reimplemened FreeLB\footnote{https://github.com/zhuchen03/FreeLB} \cite{zhu2019freelb} model, which uses the ground truth label to estimate the adversary while accumulates of gradient to speedup training. However, it requires more steps (2-5 in most cases) to achieve the best performance. 
    \item \textbf{VAT}: the virtual adversarial training\footnote{https://github.com/namisan/mt-dnn} \cite{miyato2018virtual,jiang2019smart}. It mainly leverages the dynamic model output to estimate the adversary and includes it as an additional regularizer to STD. Empirically, 1 step estimation is always enough.  
    %\hao{Is it necessary to mention SMART here. Is it because we use symmetrized KL? If so, we might need to compare with SMART too.}
    \item \textbf{STD$_{LARGE}$} the standard training objective on top of the BERT-large model (uncased) \cite{devlin2018bert}.
\end{enumerate}

First, we compare different methods on GLUE and report the standard evaluation metric on the corresponding dev set. 
As we can see from \autoref{tab:glue_dev}, {\DNAME} consistently outperforms both the standard BERT training and recent state-of-art adversarial training algorithms. Noting that on MNLI {\DNAME} obtains approximately 0.5\% improvement on average of both in/out-domain over VAT. 
More remarkably, compared with other adversarial training methods, a BERT-base model trained with the proposed TAT can even outperform the corresponding BERT-large model with standard training on several tasks by a large margin which indicates the benefit of using the global label confusion for guiding the adversarial training.  

\input{tables/zero_shot}
\input{tables/xnli}

Next, we assess the out-of-domain generalization ability of MNLI models trained with different methods by directly applying them to the test sets of HANS \cite{mccoy2019hans}, SNLI \cite{snli2015}, SciTail \cite{scitail}, and MeNLI \cite{romanov2018mednli}.
Based on the results in \autoref{tab:domain_shift}, we find that TAT can greatly improve the model robustness on out-of-domain datasets. Moreover, the MNLI model trained with TAT achieves larger improvement on two harder datasets, HANS and MedNLI, where the former is intentionally constructed to fool MNLI BERT models and the later is from the biomedical domain resulting in a significant domain shift. This further validates the effectiveness of TAT for enhancing model out-of-domain generalization.

%%%%%%%%TABLES%%%%%%%%%%%%
\subsection{XNLI}
\label{subsec:xnli}
In this section, we conduct experiments on XNLI in a zero-shot fashion to evaluate the model cross-lingual generalization. Specifically, a model is trained with the English NLI data and then directly tested on data from other languages. Following \cite{conneau2019xlmr}, our experiments are based on the pre-trained XLM-R large representations. Here, we compare our proposed TAT with a list of state-of-the-art baselines including standard training objective (XLM-R), adversarial training with XLM-R (XLM-R+R3F/R4F) \cite{aghajanyan2020rf} and another pre-train model InfoXLM \cite{chi2020infoxlm}.

Table~\ref{tab:xnli} summarizes the results on the XNLI test set. To have a fair comparison, we also report the reimplemented XLM-R \cite{conneau2018xnli} with the standard training objective (XLM-R$_{ReImp}$).
Compared with all baselines, TAT demonstrates a clear advantage on improving the model cross-lingual transferability, especially to languages that have dramatically different language topological attributes from English. Moreover, our proposed TAT advances the state-of-the-art results of XNLI to 81.7\% in terms of average accuracy over 15 languages.
%%%%%%%%Figures%%%%%%%%%%%%
\input{tables/agreement}
\subsection{Analysis}
To understand how TAT improves performance, we analyze the ambiguous samples on the MNLI dev set containing 3 classes, where each sample has 5 annotations. Based on the degree of agreement between these annotations, we divide the samples into 4 categories: 
1) \textbf{5-0-0} all five annotations are the same; 2) \textbf{4-1-0} four annotations are the same; 3) \textbf{3-2-0} three annotations are the same and the other two annotations are the same; 4) \textbf{3-1-1} three annotations are the same and the other two annotations are different.  Figure~\ref{fig:agree} reports the results. We observe that {\DNAME} outperforms the baseline consistently over all the settings. Furthermore, {\DNAME} also reduces the errors on the different samples as shown in Figure~\ref{fig:cmt}. At last, we also visualize the loss surface of {\DNAME} in Appendix~\ref{sec:lossland}.



%\input{tables/robustness}

==> 5_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
With the goal of developing more robust NLP models, a line of recent work has been devoted to identifying various kinds of superficial patterns learned by high-performance models over many popular datasets \cite{gururangan2018annotation,jia2017advsquad,mccoy2019acl}. The prevalence of data \textit{biases} over popular datasets poses a real challenge of accurately estimating the model capacity for practical applications, because a closed dataset evaluation usually inflates the model performance. This concern about dataset biases has led researchers to develop new diagnostic datasets \cite{jia2017advsquad,mccoy2019acl,nie2019adversarial} and training techniques \cite{clark2019emnlp,he2019unlearn} to overcome those discovered biases.
% In this work, we leverage two representative adversarial datasets, the Adversarial SQuAD \cite{jia2017advsquad} and HANS \cite{mccoy2019acl}, for benchmarking the model robustness towards adversarial attack.
Recent debiasing methods \cite{clark2019emnlp,he2019unlearn} require learning multiple models to access known data biases for the target dataset.
Moreover, they achieve more robust out-of-domain generalization at the price of 
in-domain performance degradation.
In contrast, we focus on the task-agnostic robust learning framework for enhancing model robustness and empirically show that regularization approaches under this framework can result in superior in-domain and out-of-domain generalization.

Training with noise has been a very popular approach for enhancing model robustness.
The dropout is a widely-used approach in deep learning to improve model generalization \cite{dropout}.
% One prominent regularization approach for deep learning is Dropout \cite{dropout},
% which has been widely used to improve model generalization. 
For adversarial learning methods, the main theme is reducing the model sensitivity toward 
small input perturbations \cite{goodfellow2014explaining, madry2017pgd},
which has been recently applied to both fine-turning \cite{jiang2019smart,pereira2020alic,zhu2019freelb,li2020textat} and pre-training \cite{liu2020alum}.
However, models trained with adversarial learning are found to have at-odd generalization \cite{tsipras2018robustness,zhang2019theoretically}. 
Our work studies robust learning methods with the goal of regularizing the model posterior difference of clean and noisy inputs.
We show that compared with the standard BERT training using dropout, robust learning methods lead to better model robustness on multiple NLP tasks.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}


\newcommand{\R}{\mathbb{R}}

\newcommand{\zeromatrix}{\mathbf{0}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mR}{\mathcal{R}}

\newcommand{\iL}{\mathit{L}}
\newcommand{\iQ}{\mathit{Q}}
\newcommand{\iR}{\mathit{R}}
\newcommand{\iU}{\mathit{U}}
\newcommand{\iV}{\mathit{V}}
\newcommand{\iX}{\mathit{X}}
\newcommand{\iY}{\mathit{Y}}

\newcommand{\sigmoid}{\text{sigm}}
%\newcommand{\vector}{\text{vec}}
\newcommand{\KL}{\text{KL}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\st}{\text{ s.t. }}

% Objective functions
\newcommand{\bilinear}[3]{#1^{\top}#2#3}
\newcommand{\bidiag}[3]{(#1 \circ #3) ^{\top} #2}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\biband}[3]{#1^{\top}#2#3}

% Dependency paths
\newcommand{\leftarc}[1]{$\leftarrow${[#1]}-}
\newcommand{\rightarc}[1]{-{[#1]}$\rightarrow$}
\newcommand{\wildcard}{$\langle*\rangle$}

\newcommand{\gene}[1]{{\texttt{#1}}}
\newcommand{\rev}[1]{#1$^{-1}$}

\newcommand{\neigh}[1]{\text{nb}\left(#1\right)}
\newcommand{\diagm}[1]{\text{diag}\left(#1\right)}
\newcommand{\ind}[1]{\mathbf{1}\left(#1\right)}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
%\newcommand{\vector}[1]{\underset{#1}{\text{vec}}}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}
\newcommand{\cheading}[2]{\textbf{#1\hfill #2}}
\newcommand{\highest}[1]{\textbf{#1}}% == highest score



%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.3mm]}
\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\etc}{\emph{etc.}\ }
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}\ }
\newcommand{\ie}{\emph{i.e.}\ }
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\rhs}{\text{ r.h.s. }}
\newcommand{\lhs}{\text{ l.h.s. }}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}
\newcommand{\tauvec}{\vec{\tau}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}

\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
\newcommand{\Img}{\ensuremath{\mathrm{Im}}}

\newcommand{\cvxCondjc}{{\sf cvxCondJC}}
\newcommand{\cvxCond}{{\sf cvxCond}}
\newcommand{\altCondjc}{{\sf altCondJC}}
\newcommand{\altCond}{{\sf altCond}}

\newcommand{\cvxDisc}{{\sf cvxDisc}}
\newcommand{\JB}{{\sf JB}}
\newcommand{\GS}{{\sf GS}}

\newcommand{\cvxJoint}{{\sf cvxJoint}}
\newcommand{\LG}{{\sf LG}}
\newcommand{\NB}{{\sf NB}}

%%%%%%%%%%%%%%%%%%%linear algebra defs%%%%%%%%%%%%%%%
\newcommand{\unifint}{\int^{1}_{0}}


==> archive/1_intro.tex <==
% !TEX encoding = UTF-8
% !TEX Root = Main.tex

\section{Introduction}
\label{sec:intro}

Although recent neural network based models have shown a great success in a wide range of natural language processing (NLP) tasks, these models may still suffer catastrophic degradation in either out-of-distribution generalization or adversarial scenarios \cite{nie2019adversarial, hsieh2019robust-self-att}. 
For example, high-accuracy sentiment classifier on a Yelp dataset can only achieve less than 10\% accuracy on a robust test \cite{jin2019bertrobust}. In addition, textual entailment models trained on MNLI \cite{mnli2018} will pick up superficial cues either focusing on the presence of certain keywords \cite{gururangan2018annotation} or whether similar words are mentioned in the sentence pairs \cite{mccoy2019acl}. Furthermore, SQuAD models achieves human-performance on in-domain data, but are very easily distracted by irrelevant sentences that contain many question words regardless of context \cite{jia2017advsquad}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/intro_fig.pdf}
    \caption{BERT-based QA and NLI model robustness towards domain shift and adversarial attack.}
    \label{fig:my_label}
\end{figure}

With the goal of developing more robust NLP models, a line of recent work has been devoted to identifying various kinds of superficial patterns learned by high-performance models over many popular datasets \cite{gururangan2018annotation,jia2017advsquad,mccoy2019acl}. The prevalence of data \textit{biases}, unintended correlations between input and output learned by statistical models, poses a real challenge of accurately estimating the model capacity for practical applications, because a closed dataset evaluation usually inflates the model performance. This concern about dataset biases has led researchers to develop new diagnostic datasets \cite{jia2017advsquad,mccoy2019acl,nie2019adversarial} and training techniques \cite{clark2019emnlp} to overcome those discovered biases. However, typical debiasing methods \cite{clark2019emnlp,he2019unlearn} not only requires learning multiple models with accesss to known data biases for the target dataset but achieves more robust out-of-domain generalization at the price of in-domain performance drop.
Instead of relying on the knowledge of dataset bias or expensive data sampling strategies, we focus on task-agnostic training techniques for enhancing model robustness, \ie achieving good generalization for both in-domain and out-of-domain datasets.



Motivated by recent success of adversarial training in computer vision \cite{madry2017pgd,goodfellow2014explaining} and NLP \cite{zhu2019freelb,jiang2019smart,cheng-etal-2019-adv-nmt,wang2019adv-lm},
we propose a robust learning framework, directly regularizing the model posterior discrepancy for clean and noisy inputs, as a means to enhance the model robustness.
Here, we first provide a theoretical connection of two recent methods under this framework, Virtual Adversarial Training (VAT) \cite{madry2017pgd} and Jacobian Regularization (JR) \cite{sokilic2017TSP}.
Furthermore, we show that an alternative regularizer, posterior discrepancy minimization (PDM) based on KL-divergence, is also a theoretically justified approach with reduced computational complexity and a great potential for large-scale neural models for either fine-tuning or pretraining large-scale language model such as BERT \cite{devlin2018bert} or GPT \cite{gpt22019}.

Given large-scale pretrained neural language models demonstrate superior for both in-domain \cite{devlin2018bert,liu2019roberta} and out-of-domain generalization \cite{hendrycks2020acl}, this work systematically studies the robust learning framework on top of BERT \cite{devlin2018bert} over a diverse set of tasks in terms of both in-domain and out-of-domain generalization. \xiaodl{we may need to mention that it can be applied to other nlp models.} First, we train and evaluate the corresponding sentiment analysis, textual entailment and question answering (QA) models on the matched datasets \cite{sst2013,mnli2018,squad1,squad2}.
Then, the trained QA model and the sentiment analysis model are applied directly on a biomedical QA dataset, BioASQ \cite{bioasq}, from MRQA \cite{mrqa2019} and IMDB movie review dataset \cite{imdb2011} respectively for evaluating the model robustness towards domain shift. Finally, we consider direct evaluations with two challenge adversarial datasets \cite{jia2017advsquad,mccoy2019acl} which were designed to pool models that leverage superficial strategies for textual entailment and QA respectively.

Based on our experiments, we show that the robust learning through regularizing the posterior discrepancy for clean and noise inputs is very effective for improving model generalization for both supervised and semi-supervised learning settings. Compared with JR, models trained with VAT and PDM achieve better improvement which indicates the advantage of incorporating model confidence to adapt the regularization based on our theoretical analysis. Models trained with VAT achieve the best in-domain generalization and robustness towards adversarial attacks. In addition to being computationally more efficient, PDM achieves consistent improved generalization, especially towards domain difference caused by topic and style shift, indicating its great potential for enhancing the robustness of large-scale neural models.
\eat{
In summary, we make the following contributions:
    \begin{itemize}
        \item Based on the view of robust learning through penalizing the posterior difference between clean and perturbed inputs, we establish a theoretical connection between VAT and JR, which are two recently proposed training techniques under this framework. Motivated by the observation, we further propose a simple and effective method, PDM, to regularize the model stability with a  theoretical justification.
        \item To best our knowledge, we are the first to apply those robust learning techniques on top of BERT to systematically study their effectiveness in terms of in-domain generalization and \textit{zero-shot} out-of-domain generalization including both domain shift and adversarial attack scenarios. Compared with vanilla BERT training across a diverse set of QA and sentence classification tasks, we show that robust learning achieves significant improvement for both in-domain and out-of-domain evaluations which indicates its great potential in enhancing model robustness.
    \end{itemize}
    }


\eat{Generalization and robustness are two fundamental considerations in assessing machine learning methods.
Ideally, a learned model should perform well on unseen test examples and withstand adversarial attacks.
In natural language processing (NLP), pre-training neural language models on unlabeled text has proven very effective to improve generalization performance for a variety of downstream tasks, as exemplified by BERT \cite{devlin2018bert} and other transformer-based models \cite{liu2019roberta,gpt22019,clark2020electra,dong2019unified, bao2020unilmv2}. 
However, these models may still suffer catastrophic failures in adversarial scenarios \cite{nie2019adversarial, hsieh2019robust-self-att}. 
For example, \newcite{jin2019bertrobust} show that classification accuracy on a Yelp dataset drops from 95.6\% on standard test to 6.8\% on robust test for a BERT model. 


Adversarial training \cite{madry2017pgd,goodfellow2014explaining} has been well studied in computer vision, but past work shows that it often hurts generalization \cite{raghunathan2019adv-hurt,min2020curious}.
In NLP, there is growing interest in adversarial training, but existing work typically focuses on assessing the impact on generalization  \cite{zhu2019freelb,jiang2019smart,cheng-etal-2019-adv-nmt,wang2019adv-lm}. 

Moreover, adversarial training is generally limited to task-specific fine-tuning\footnote{A notable exception is \newcite{wang2019adv-lm}, but it only applied adversarial training to generative language modeling.}. See \newcite{minaee2020deepreview} for a recent survey.

In this paper, we present the first comprehensive study on adversarial pre-training, and show that it can improve both generalization and robustness for a wide range of NLP tasks.
We propose a unifying algorithm {\DNAME} (\textbf{A}dversarial training for large neural \textbf{L}ang\textbf{U}age \textbf{M}odels), which augments the standard training objective with an additional term that maximizes the adversarial loss via applying perturbation in the embedding space.
{\DNAME} is generally applicable to pre-training and fine-tuning, on top of any Transformer-based language models. 

We conduct a comprehensive evaluation on various NLP tasks across multiple benchmark datasets, including GLUE, SQuAD v1.1/v2.0, SNLI, SciTail for assessing model generalization, and ANLI, HELLSWAG, SWAG, Adversarial SQuAD for assessing model robustness.   
Experimental results show that by conducting adversarial pre-training, {\DNAME} attains significant improvements, often outperforming previous state of the art by a large margin.
This is true even for the extremely well-trained RoBERTa model, where continual pre-training without adversarial training fails to attain any gain.

Remarkably, in addition to improving generalization, we find that adversarial pre-training also substantially improves robustness, as exemplified by the resulting large gains in adversarial datasets such as ANLI, Adversarial-SQuAD, HELLASWAG, which significantly reduces the gap between standard errors and robust errors for popular models like BERT and RoBERTa. This suggests that adversarial training on unlabeled data can provide a promising direction to reconcile the apparent conflict between generalization and robustness as observed in prior work \cite{raghunathan2019adv-hurt,min2020curious}.
We also show that adversarial pre-training can be combined with adversarial fine-tuning, resulting in extra gains. 

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose {\DNAME}, a general algorithm to incorporate adversarial training for pre-training and fine-tuning large neural language models.
    \item We conduct a comprehensive evaluation on a wide range of NLP tasks and assess the impact of adversarial training in pre-training from scratch, continual pre-training, task-specific fine-tuning, and their combinations.
    \item We obtain significant improvements over prior state of the art, including extremely well-trained models such as RoBERTa, in both generalization and robustness.
    \item To facilitate research, we will release our code and pre-trained models.
\end{itemize}
}



==> archive/4_0_setting.tex <==
\eat{
 In this section, we start with an introduction to the dataset used for pre-training and downstream tasks used for evaluation. Second, we study both model generalization and model robustness of the proposed model {\DNAME} and compare it with state-of-the-art models including BERT and RoBERTa. We then apply {\DNAME} with adversarial fine-tuning to further showcase more improvements by adversarial training.  

\subsection{Datasets and Benchmarks}
\label{subsec:dataset}
\textbf{Pre-training dataset:} 

We collect three publicly available large-scale raw corpora in total of 82G words. They are:
\begin{itemize}
    \item Wikipedia is an English Wikipedia dump which contains 13G raw text after cleaning \footnote{https://dumps.wikimedia.org/enwiki/}. It is originally used for BERT training. \vspace{-1mm}
    \item OPENWEBTEXT \cite{Gokaslan2019OpenWeb} is a large text corpus of 38G words. It is extracted from the publicly available URL on Reddit. \vspace{-1mm}
    \item STORIES %is used firstly by \cite{trinh2018simple} which 
    is a subset of CommonCrawl data developed by \citet{trinh2018simple} for commonsense reasoning (Winograd schemas).
    % pre-training \cite{trinh2018simple}. 
    It contains 31G words. \vspace{-1mm}
\end{itemize}


\noindent\textbf{Downstream benchmarks:} 
To evaluate model generalization, we use the well-known GLUE \cite{wang2018glue} and SQuAD (v1.1 and v2.0) \cite{squad1,squad2} benchmarks and three named entity recognition (NER) tasks in biomedical domain.
To evaluate models' robustness to adversarial attack, we use the ANLI~\cite{nie2019adversarial}, 
adversarial SQuAD~\cite{jia2017advsquad} and 
HELLASWAG~\cite{zellers2019hellaswag} datasets. 
We use two repres entative benchmarks, MNLI~\cite{mnli2018} (in GLUE) and ANLI \cite{nie2019adversarial}, in the adversarial fine-tuning experiments, combined with three additional datasets: SWAG~\cite{zellers2018swag}, SNLI~\cite{snli2015} and SciTail~\cite{scitail}. 
These benchmarks cover a wide range of NLP tasks including classification, ranking, regression, machine reading comprehension, and named entity recognition. A detailed description these datasets is provided in Appendix~\ref{sec:appendix}.

\subsection{Implementation Details}
\label{subsec:details}
We perform three types of training tasks in our experiments: pre-training from scratch, continual pre-training on a well-trained model, and task-specific fine-tuning.

We pre-train BERT models from scratch using the Wikipedia corpus \footnote{BookCorpus is no longer publicly available.}. 
The training code is based on Megatron, implemented in PyTorch  \cite{shoeybi2019megatron}
\footnote{https://github.com/NVIDIA/Megatron-LM}.  
ADAM \cite{kingma2014adam} is used as the optimizer with a learning rate of $1\times 10^{-4}$ which firstly firstly schedules 1\% steps warmup and then decays linearly. 
Following \citet{devlin2018bert}, the model is updated for 1M steps with a batch size of 256.
We set the perturbation size $\epsilon=1\times 10^{-5}$, the step size $\eta=1\times10^{-3}$, and the variance of normal distribution $\sigma=1\times10^{-5}$. 
Since the loss is dominated by the first term in Eq~\ref{eq:alum}, we set $\alpha=10$, and $K=1$ for training efficiency. 
The training takes 10 days on one DGX-2 machine with 16 V100-32G GPUs.

For continual pre-training on RoBERTa \cite{liu2019roberta}, 
we use RoBERTa's default training parameters, except a smaller learning rate ($4\times10^{-5}$), and run for 100K training steps with a batch size of 256 on the corpora of 82G text. 
The code is implemented with FairSeq\footnote{https://github.com/pytorch/fairseq}. 
The training takes 7 days on two DGX-2 machines.

For fine-tuning with and without adversarial training,
we use the open-sourced toolkit \cite{liu2020mtmtdnn,liu2015mtl} \footnote{https://github.com/namisan/mt-dnn}. 

We use ADAM \cite{kingma2014adam} and RADAM \cite{liu2019radam} as our optimizers with learning rates of $\{5\times 10^{-6}, 8 \times 10^{-6}, 1\times 10^{-5}, 2\times 10^{-5}\}$.   
A linear learning rate decaying schedule with a warm-up of $0.1$ is applied to all the tasks, unless stated otherwise. 
The batch size is set to 16, 32 or 64.  
We set the dropout rate to $0.1$ for all the task-specific layers, except $0.3$ for MNLI and $0.05$ for CoLA. 
To avoid gradient exploding, we clip the gradient norm within $1$.  
All the texts are tokenized using WordPiece and chopped to spans up to $512$ tokens. 
We fine-tune the model for up to 10 epochs with the provided task-specific training set and pick the best task-specific model based on its performance on the dev set.}


==> archive/vat_jacobian.tex <==

% Overview.
In this section, we first introduce the robust learning framework that regularizes the difference of posterior between clean and noisy inputs.
Based on this framework, we set up the basic notions of two recent methods, \ie VAT and JR, and show their theoretical connection.
Finally, we provide an alternative regularization approach that achieves robustness by directly minimizing the posterior discrepancy.
In the following, we use $f_\Theta(\xvec):\RR^n\to\RR^m$ to denote the posterior function,
which is a neural network parameterized by $\Theta$ that maps the input $\xvec\in\RR^n$ to the output probability space with $m$ discrete classes.

Both adversarial learning \cite{goodfellow2014explaining} and robust learning aim at making the model more robust.
Adversarial learning focuses on minimizing the following objective
\begin{eqnarray}
\min_\Theta \max_{\|\epsilon\|=1} L(f_\Theta(\xvec+c\epsilon), y),
\end{eqnarray}
where $L$ is the cross-entropy loss, $\epsilon\in\RR^n$ is a random vector bounded by a norm, $c$ is a small positive constant and $\yvec$ is the target label.
The robust learning directly regularizes the model local smoothness, \eg stabilizing the model posterior distribution towards small input perturbations.
Typically, it is in the form of 
\begin{eqnarray}
\min_\Theta L(f_\Theta(\xvec), \yvec) + \alpha R(f_\Theta(\xvec), f_\Theta(\hat{\xvec})),
\end{eqnarray}
where $\hat{\xvec} = \xvec + c\epsilon$, $R$ is a regularization term promoting the model stability, and $\alpha$ is a hyperparameter for balancing the classification loss and the regularization term.
As we can see, robust learning is a task-agnostic regularization which makes it applicable to semi-supervised, self-supervised and unsupervised learning.
For simplicity, we will use $f$ and $R$ to denote $f_\Theta$ and $R(f_\Theta(\xvec), f_\Theta(\hat{\xvec}))$, respectively.
In the following, we show three realizations of $R$.%\xiaodl{Need a citation.}

\subsection{Jacobian Regularization}
\label{ssec:jacobian}
A recent robust learning approach to stabilize the model is Jacobian regularization  \cite{sokilic2017TSP}.
Specifically, using the input-output Jacobian matrix, $J=J_f(\xvec)\in\RR^{m\times n}$, 
we can get the first-order Taylor approximation
\begin{equation}
    f(\xvec + c\epsilon) = f(\xvec) + c\epsilon J_f(\xvec).
\end{equation}
In order to reduce the overall model sensitivity to the input perturbation, \citet{sokilic2017TSP} propose to directly regularize the Frobenius norm of the input-output Jacobian matrix so that
\begin{eqnarray}
\label{eqn:jacobian_norm}
\nonumber
\|f(\xvec+c\epsilon) - f(\xvec)\|_2^2 & = & \|c\epsilon J\|_2^2\\
& \leq& c^2 \|\epsilon\|_2^2 \|J\|_F^2,
\end{eqnarray}
where $\|\cdot\|_2$ is the $L2$ norm, and $\|J\|^2_F=\tr(J^TJ)$ is the Frobeinus norm of the Jacobian matrix with $\tr$ as the trace operator.
In other words, by letting $R = \|J\|^2_F$, the $L2$ difference between clean and noisy inputs is thus being effectively regularized.

\subsection{Virtual Adversarial Training}
Motivated by the adversarial learning objective used in \cite{goodfellow2014explaining}, \citet{miyato2018virtual} introduce a regularized objective to enhance the model robustness towards small input perturbations 
\begin{align}
\label{eqn:vat}
    \min [L(\yvec, \hat{\yvec}) + \alpha\underbrace{\max_{\|\epsilon\|=1} D(\hat{\yvec}, f(\xvec+c\epsilon))}_{R}],
\end{align}
where $D$ is the KL divergence, and $\hat{\yvec}=f(\xvec)$. 
Based on the above definition, VAT essentially regularizes the worst-case posterior difference between the clean and noisy input using an inner loop to search for the most anisotropic direction.

Although sharing with JR the same spirit of encouraging the local smoothness of the model, VAT does not have a theoretical justification yet.
In what follows, we draw the theoretical connection between these two methods and 
show that VAT is a regularization upper bound for JR.

\subsection{Connection between VAT and JR}
Here, we show that VAT and JR can be directly related through the definition of induced matrix norm.
Specifically, the matrix norm of the Jacobian matrix is
\begin{eqnarray}
\|J\| = \sup_{\|\nu\|=1} \|J\nu\|,
\end{eqnarray}
where the matrix norm on the left side is induced by the corresponding vector norm on the right side.
It is easy to show that
\begin{eqnarray*}
c^2\|J\|_F^2 & \leq & m c^2 \|J\|_\infty^2 \\
& = & m \sup_{\|\epsilon\|_\infty=1} \|c\epsilon J\|_\infty^2 \\
& = & m \sup_{\|\epsilon\|_\infty=1} \|f(\xvec + c\epsilon)-f(\xvec)\|_\infty^2 \\
& \leq & m \sup_{\|\epsilon\|_\infty=1} \|f(\xvec + c\epsilon)-f(\xvec)\|_1^2 \\
& \leq & 2m \sup_{\|\epsilon\|_\infty=1}D(f(\xvec), f(\xvec + c\epsilon)),
\end{eqnarray*}
where $m$ is the number of classes, and the last inequality is attained based on the Pinsker's inequality.
Given $\|{\bm \nu}\|_2\leq\|{\bm \nu}\|_1$, it is straightforward to extend the relation for L2 norm with proper scaling. It is equivalent to the maximization defined in \autoref{eqn:vat} when $L_\infty$ norm is used.
Therefore, the VAT regularization provides an upper bound for the Frobenius norm of the Jacobian matrix.

Although both VAT and JR have been shown to effectively enhance model robustness, they are both computationally expensive. For VAT, even the perturbation is estimated by only one step optimization, it requires 3 forward passes and 2 back-propagations, approximately tripling the computation.
% On the other hand, Jacobian regularization has been shown to effectively improve the model robustness toward adversarial attacks \cite{sokilic2017TSP} for computer vision tasks.
% However, it is not clear whether the technique can be useful for improving model robustness for NLP tasks.
% Moreover, the computational cost of Jacobian regularization linearly depends on the number of classes.
For JR, the computational cost linearly scales with the number of classes.
For tasks where the output space is large such as extractive QA and language model pretraining, it is computationally prohibitive to use this technique.
Moreover, despite of its success in computer vision tasks \cite{sokilic2017TSP}, 
it is unclear whether JR can also improve model robustness for NLP tasks.


\subsection{Posterior Discrepancy Minimization}
\label{ssec:pdm}
Given the high computational demand of JR and VAT, a natural question is whether we can directly regularize the posterior difference between the outputs of clean and noisy inputs. 
Instead of searching for the most anisotropy as VAT, we show that 
the PDM is also a theoretically justified approach and provides an approximation to JR.

Specifically, we consider using the KL divergence, \ie
\begin{align}
D(f(\hat{\xvec}), f(\xvec)) = \sum_i &
    f_i(\hat{\xvec}) \log {f_i(\hat{\xvec}) \over f_i(\xvec)},
\end{align}
where $\hat{\xvec} = \xvec + \epsilon$ and $f_i$ indicates the $i$-the element of vector $f$.
The first and second derivatives of $D$ with regard to $\epsilon$ are
\begin{align*}
D' & =  \sum_i f'_i(\hat{\xvec})\log(d_i) + f'(\hat{\xvec}),\\
D''& =  \sum_i f''_i(\hat{\xvec})\log(d_i) +
{f'_i(\hat{\xvec})^2 \over f_i(\hat{\xvec})} + f''_i(\hat{\xvec}),
\end{align*}
where $d_i = {f_i(\hat{\xvec}) \over f_i(\xvec)}$.
Let $D(\epsilon) = D(f(\hat{\xvec}), f(\xvec)))$.
When evaluating at $0$,  
the second order approximation of the KL divergence is
\begin{eqnarray*}
D(\epsilon) 
& = & D(0) + \epsilon D'(0) + {\epsilon^2 D''(0) \over 2}\\
& = & \sum_i (\epsilon f'_i + \epsilon^2{{f'}^2_i \over 2f_i} + \epsilon^2 {f_i''\over 2}) \\
& = & \sum_i \epsilon^2{{f'}^2_i \over 2f_i} 
% \label{eqn:weighted_frob_norm}
% & = & J^T\text{diag}({\epsilon^2 \over f})J,
\end{eqnarray*}
where $\sum_i f'_i=(\sum_i f_i)'=(1)'=0$ and similarly $\sum_i f''_i=0$.

Since the perturbation is typically a Gaussian noise, $\epsilon \thicksim\mathcal{N}(0, c^2I)$,
we take the expectation for the above equation
\begin{eqnarray}
\EE_\epsilon [D(\hat{\xvec}, \xvec)] & =& \EE_\epsilon [\sum_i \epsilon^2{{f'}^2_i \over 2f_i}]\\
& = & \sum_i {{f'}^2_i \over 2f_i} \EE_\epsilon [\epsilon^2] \\
\label{eqn:weighted_frob_norm}
& = & {c^2\over 2}J^T\diag{1 \over f} J,
\end{eqnarray}
where $J$ is the input-output Jacobian of $f$, $\text{diag}({1 \over f})$ is a diagonal matrix with its diagonal elements equal to the vector ${1 \over f}$, 
Comparing with $\|J\|^2_F=\tr(J^TJ)$, \autoref{eqn:weighted_frob_norm} can be seen as a weighted version of JR where each row is rescaled by the model confidence $f_i$ for the corresponding class.
In other words, it is closer to JR for more confident classes,
whereas for uncertain classes it allows less Jacobian variance. 
Additionally, it's easy to show that the reversed KL divergence also provides the same approximation.

Although this alternation has been suggested in \cite{miyato2018virtual}, we are the first to show that PDM has a theoretical justification and that training with both VAT and PDM provides an approximation to a variant of JR which adapts the regularization based on model confidence.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/robustness.tex <==
\begin{table*}[htb!]
    \centering
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
\toprule    
         \multirow{2}{*}{Model} & \multicolumn{4}{c|}{Dev} & \multicolumn{4}{c}{Test}  \\
         \cline{2-9}
          &  R1 & R2 & R3 & All & R1 & R2 & R3 & All  \\
          \hline 
 		%\multicolumn{9}{c}{ MNLI + SNLI + ANLI + FEVER  }  \\ \hline
 BERT\textsubscript{BASE}&55.7&46.3&43.4 &48.2 &55.1 &45.0 &43.1 & 47.4\\
%\alumbert{} &62.0&48.6&48.1 & \textbf{52.6} &61.3 &45.9 &44.3 & \textbf{50.1}\\ 
TAT &59.9&47.1&44.7 &  & & & & \textbf{50.1}\\ 

\bottomrule
    \end{tabular}
    \caption{Comparison of standard and adversarial training on the adversarial dataset ANLI. R1, R2 and R3 are rounds with increasing difficulty.}
    \label{tab:anli_full}
\end{table*}
